Unsupervised Time Series Outlier Detection with Diversity-Driven Convolutional Ensembles -- Extended Version

With the sweeping digitalization of societal, medical, industrial, and scientific processes, sensing technologies are being deployed that produce increasing volumes of time series data, thus fueling a plethora of new or improved applications. In this setting, outlier detection is frequently important, and while solutions based on neural networks exist, they leave room for improvement in terms of both accuracy and efficiency. With the objective of achieving such improvements, we propose a diversity-driven, convolutional ensemble. To improve accuracy, the ensemble employs multiple basic outlier detection models built on convolutional sequence-to-sequence autoencoders that can capture temporal dependencies in time series. Further, a novel diversity-driven training method maintains diversity among the basic models, with the aim of improving the ensemble's accuracy. To improve efficiency, the approach enables a high degree of parallelism during training. In addition, it is able to transfer some model parameters from one basic model to another, which reduces training time. We report on extensive experiments using real-world multivariate time series that offer insight into the design choices underlying the new approach and offer evidence that it is capable of improved accuracy and efficiency. This is an extended version of "Unsupervised Time Series Outlier Detection with Diversity-Driven Convolutional Ensembles", to appear in PVLDB 2022.

==> figures/Old/Old_figures.tex <==
\begin{figure}[ht!]
  \centering
  \begin{tikzpicture}
  \begin{axis}[
    width=0.5*\linewidth,
    height=0.6*\axisdefaultheight,
	ylabel={},
	yticklabel style={
    /pgf/number format/fixed,
    /pgf/number format/precision=5},
    scaled y ticks=false,
    symbolic x coords={ROC,PR},
    xtick=data,
	enlargelimits=0.4,
	legend style={at={(0.5,-0.25)},
	anchor=north,legend columns=-1},
	ybar]
    \addplot coordinates {(ROC,0.587827821) (PR,0.794171999)};
    \addplot coordinates {(ROC,0.572612149) (PR,0.804207261)};
    \legend{Clean,Outliers}
    \end{axis}
    \end{tikzpicture}
  \caption{Effect on metrics of using a clean data or not during the training stage.}
  \label{fig:thresholdChoice2}
\end{figure}


\begin{figure}[ht!] 
\small
\centering 
    \begin{subfigure}[b]{0.48\linewidth}
    \begin{tikzpicture}
        \begin{axis}[
            % xlabel=Ensemble Components,
            xlabel=\# of Basic Models,
            width=\linewidth,
            height=0.6*\axisdefaultheight,
            legend style={at={(1.32,1.26)},anchor=north,legend columns=-1}]
            \addplot[purple, mark=triangle] table[x=t, y=a] {figures/metricsDonut.dat};
            \addlegendentry{\textit{Precision}}
            \addplot[green, mark=square] table[x=t, y=b] {figures/metricsDonut.dat};
            \addlegendentry{\textit{Recall}}
            \addplot[blue, mark=star] table[x=t, y=c] {figures/metricsDonut.dat};
            \addlegendentry{\textit{F1}}
            \end{axis}
        \end{tikzpicture}
        \caption{\textit{Donut}} \label{subfig:donut}  
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
            % xlabel=Ensemble Components,
            xlabel=\# of Basic Models,
            width=\linewidth,
            height=0.6*\axisdefaultheight,
            legend style={at={(0.5,-0.4)},anchor=north,legend columns=-1}]
            \addplot[purple, mark=triangle] table[x=t, y=a] {figures/metricsSMD.dat};
            \addplot[green, mark=square] table[x=t, y=b] {figures/metricsSMD.dat};
            \addplot[blue, mark=star] table[x=t, y=c] {figures/metricsSMD.dat};
            \end{axis}
        \end{tikzpicture}
    \caption{\textit{SMD}} \label{subfig:SMD}  
    \end{subfigure}
\caption{Accuracy Evolution.}% according to the number of ensemble components.}
\label{fig:metricsEvolution}
\end{figure}


\begin{figure}[ht!]
\small
\centering 
  \begin{subfigure}[b]{0.48\linewidth}
  \begin{tikzpicture}
    \begin{axis}[
        xlabel=\% of k,
        x dir=reverse,
        width=\linewidth,
        height=0.6*\axisdefaultheight,
        ytick={0.98,0.99,1},
        legend style={at={(1.32,1.26)},anchor=north,legend columns=-1}]
        \addplot[purple, mark=triangle] table[x=t, y=a] {figures/Donut_K.dat};
        \addlegendentry{\textit{Precision}@$K$}
        \addplot[green, mark=square] table[x=t, y=b] {figures/Donut_K.dat};
        \addlegendentry{\textit{Recall}@$K$}
        \addplot[blue, mark=star] table[x=t, y=c] {figures/Donut_K.dat};
        \addlegendentry{\textit{F1}@$K$}
        \end{axis}
    \end{tikzpicture}
    \caption{\textit{Donut}} \label{subfig:donutK}  
  \end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
  \begin{tikzpicture}
    \begin{axis}[
        xlabel=\% of k,
        x dir=reverse,
        width=\linewidth,
        height=0.6*\axisdefaultheight,
        legend style={at={(0.5,-0.4)},anchor=north,legend columns=-1}]
        \addplot[purple, mark=triangle] table[x=t, y=a] {figures/SMD_K.dat};
        %\addlegendentry{Precision@K}
        \addplot[green, mark=square] table[x=t, y=b] {figures/SMD_K.dat};
        %\addlegendentry{Recall@K}
        \addplot[blue, mark=star] table[x=t, y=c] {figures/SMD_K.dat};
        %\addlegendentry{F1@K}
        \end{axis}
    \end{tikzpicture}
\caption{\textit{SMD}} \label{subfig:SMDK}  
\end{subfigure}
\caption{Accuracy Evolution for Top-$K$ Percent of Outliers}%according to the percentage of required outliers for Donut and SMD datasets.}
\label{fig:topK}
\end{figure}  


\begin{figure}[ht!]
  \centering
  \begin{tikzpicture}
    \begin{axis}[
        xlabel=Epochs,
        width=0.5*\linewidth,
        height=0.6*\axisdefaultheight,
        legend style={at={(0.5,-0.4)},anchor=north,legend columns=-1}]
        \addplot[purple, mark=triangle] table[x=t, y=a] {figures/metricsAIOps.dat};
        \addlegendentry{\textit{Precision}}
        \addplot[green, mark=square] table[x=t, y=b] {figures/metricsAIOps.dat};
        \addlegendentry{\textit{Recall}}
        \addplot[blue, mark=star] table[x=t, y=c] {figures/metricsAIOps.dat};
        \addlegendentry{\textit{F1}}
        \end{axis}
    \end{tikzpicture}
  \caption{Metrics evolution according to the epochs of training for the \textit{AIOps} dataset. They are relatively stable over time.}
  \label{fig:epochsAIOps}
\end{figure}


\begin{figure}[ht!]
\small
  \centering
  \begin{tikzpicture}
      \begin{axis}[
        	ybar, ymode = log,
        	ymin =3,
        	bar width=8pt,
            width=\linewidth,
            height=0.8*\axisdefaultheight,
        	yticklabel style={},
        	xtick align=inside,
        	ylabel=Runtime in minutes ($\mathit{log}$),
            xtick = data,
            symbolic x coords={\textit{AIOps},\textit{ECG},\textit{Donut},\textit{SMD}},
        	enlargelimits=0.2,
        	legend style={at={(0.5,-0.15)},
        	anchor=north,legend columns=2}]
        	\addplot [YellowGreen!20!black,fill=YellowGreen!80!white] coordinates {(\textit{AIOps},560) (\textit{ECG},12) (\textit{Donut},30) (\textit{SMD},140)};
            \addplot [Mulberry!20!black,fill=Mulberry!80!white] coordinates {(\textit{AIOps},7) (\textit{ECG},1.1) (\textit{Donut},1.5) (\textit{SMD},3.5)};
            \addplot [Melon!80!white,fill=Melon!80!white] coordinates {(\textit{AIOps},1500) (\textit{ECG},25)
        	(\textit{Donut},150) (\textit{SMD},400)};
        	\addplot [MidnightBlue!80!white,fill=MidnightBlue!80!white] coordinates {(\textit{AIOps},54) (\textit{ECG},12)
        	(\textit{Donut},8) (\textit{SMD},56)};
            \legend{\textit{RAE},\textit{CAE},\textit{RAE-Ensemble},\textit{CAE-Ensemble}}
        \end{axis}
    \end{tikzpicture}
  \caption{Execution Time Comparison.}% (in minutes) between the Neural Network based models in the logarithm scale. SMD, Donut, and ECG are multiples series, while AIOps is a single one.}
  \label{fig:executionTime}
%  \vspace{-10pt}
\end{figure}

\begin{figure}[ht!]
\small
  \centering
    \begin{subfigure}[b]{0.48\linewidth}
      \begin{tikzpicture}
      \begin{axis}[
        ybar,
        width=\linewidth,
        height=0.6*\axisdefaultheight,
    	ylabel={},
    	yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5},
        scaled y ticks=false,
        symbolic x coords={\textit{ROC},\textit{PR}},
        xtick=data,
        xtick align=inside,
    	enlargelimits=0.4,
        legend style={at={(1.3,1.26)},
    	anchor=north,legend columns=2}]
    	\addplot coordinates {(\textit{ROC},0.781256977) (\textit{PR},0.973127242)};
    	\addplot coordinates {(\textit{ROC},0.872532399) (\textit{PR},0.986306077)};
        \legend{Aggregated, Last}
        \end{axis}
        \end{tikzpicture}
        \caption{\textit{AIOps}} \label{subfig:AIOps}  
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
          \begin{tikzpicture}
      \begin{axis}[
        ybar,
        width=\linewidth,
        height=0.6*\axisdefaultheight,
    	ylabel={},
    	yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5},
        scaled y ticks=false,
        symbolic x coords={\textit{ROC},\textit{PR}},
        xtick=data,
        xtick align=inside,
    	enlargelimits=0.4,
        legend style={at={(0.5,1.45)},
    	anchor=north,legend columns=1}]
    	\addplot coordinates {(\textit{ROC},0.647288014) (\textit{PR},0.913661777)};
    	\addplot coordinates {(\textit{ROC},0.670769814) (\textit{PR},0.939487123)};
        \end{axis}
        \end{tikzpicture}
        \caption{\textit{ECG}} \label{subfig:ECG}  
    \end{subfigure}
  \caption{Sensitivity Analysis to  Ensemble  Mechanism} %Effect on metrics for using an aggregated ensemble against the last trained model on the univariate and multivariate datasets.}
  \label{fig:ensembleType}
\end{figure}

\begin{figure}[ht!]
  \centering
    \begin{tikzpicture}
        \begin{axis}[ xbar,
        xmin=-0.002,
        xmax=0.002,
        width=\linewidth,
        height=0.6*\axisdefaultheight,
        enlarge y limits=1,
        enlarge x limits=0.08,
        xlabel={Differences},
        ylabel={},
        symbolic y coords={\textit{Precision},\textit{Recall},\textit{F1}},
        ytick=\empty,
        xticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5},
        scaled x ticks=false,
        legend style={at={(0.5,-0.4)},
        anchor=north,legend columns=-1},]
        \addplot [Peach!20!black,fill=Peach!80!white] coordinates{(-0.000878089,Precision)};
        \addplot [SeaGreen!20!black,fill=SeaGreen!80!white] coordinates{(0.001855074,Recall)};
        \addplot [Orchid!20!black,fill=Orchid!80!white] coordinates{(0.000458738,F1)};
        \legend{\textit{Precision}, \textit{Recall}, \textit{F1}}
        \end{axis}
    \end{tikzpicture}
  \caption{Effect on metrics for using an average ensemble against the last trained model on the univariate and multivariate. A positive value means that the last trained model is better than the average one.}
  \label{fig:ensembleTypeOld}
\end{figure}

\begin{figure}[ht!]
  \centering
\begin{tikzpicture}

\node (X1) at (-2.5,0) {$X_{t-2}$};
\node (X2) at (-1.25,0) {$X_{t-1}$};
\node (X3) at (0,0) {$X_{t}$};
\node (X4) at (1.25,0) {$X_{t+1}$};
\node (X5) at (2.5,0) {$X_{t+2}$};

\node[left of=X1] (left) {\phantom{$X_t$}};
\node[right of=X5] (right) {\phantom{$X_t$}};

\begin{scope}[->,rounded corners=5pt,thick]

\draw ([yshift=7pt]left.north) -| (X1.north);
\draw ([yshift=-7pt]left.south) -| (X2.south);
\draw ([xshift=4pt]X1.north) -- ([xshift=4pt,yshift=7pt]X1.north)
  -| ([xshift=-4pt]X3.north);
\draw ([xshift=4pt]X2.south) -- ([xshift=4pt,yshift=-7pt]X2.south)
  -| ([xshift=-4pt]X4.south);
\draw ([xshift=4pt]X3.north) -- ([xshift=4pt,yshift=7pt]X3.north)
  -| ([xshift=-4pt]X5.north);
\draw ([xshift=4pt]X4.south) -- ([xshift=4pt,yshift=-7pt]X4.south)
  -- ([yshift=-7pt]right.south);
\draw ([xshift=4pt]X5.north) -- ([xshift=4pt,yshift=7pt]X5.north)
  -- ([yshift=7pt]right.north);

\draw (X1.east) -- (X2.west);
\draw (X2.east) -- (X3.west);
\draw (X3.east) -- (X4.west);
\draw (X4.east) -- (X5.west);
\draw (left.west) -- (X1.west);
\draw (X5.east) -- (right.east);

\end{scope}

\end{tikzpicture}
  \caption{Sequence-to-sequence process, considering a temporal dependency for the previous two elements.}
  \label{fig:sequentialProcess}
\end{figure}

\begin{figure}[ht!]
  \centering
    \begin{tikzpicture}[
    plain/.style={draw=none},
    labels/.style={draw=none,rectangle,inner sep=5pt,minimum width=4em},
    net/.style={matrix of nodes,
      nodes={draw,line width=1.0pt,circle,inner sep=5pt},
      nodes in empty cells,row sep=-2pt}]
    \matrix[net] (mat)
    { & |[plain]| & & |[plain]| &\\
      |[plain]| & & |[plain]| & & |[plain]| &\\
      & |[plain]| & & |[plain]| &\\
      |[plain]| & & |[plain]| & & |[plain]| &\\
      & |[plain]| & & |[plain]| &\\
      |[plain]| & |[plain]| \\
    |[labels]| & |[labels]| & |[labels]| & |[labels]| & |[labels]| & |[labels]| \\ };
    \foreach \ai in {1,3,5} {
      \draw[line width=1.0pt,->] (mat-\ai-1) -- (mat-2-2);
      \draw[line width=1.0pt,->] (mat-\ai-1) -- (mat-4-2);
    }
    \draw[line width=1.0pt,dashed,->] (mat-1-3) -- (mat-2-4);
    \draw[line width=1.0pt,dashed,->] (mat-3-3) -- (mat-4-4);
    \draw[line width=1.0pt,dashed,->] (mat-5-3) -- (mat-2-4);
    \draw[line width=1.0pt, double,->] (mat-1-5) -- (mat-2-6);
    \draw[line width=1.0pt, double,->] (mat-3-5) -- (mat-2-6);
    \draw[line width=1.0pt, double,->] (mat-5-5) -- (mat-4-6);
    \node[fit=(mat-7-1)(mat-7-2)]{(a) Full connected};
    \node[fit=(mat-7-3)(mat-7-4)]{(b) Random choice};
    \node[fit=(mat-7-5)(mat-7-6)]{(c) Data-driven};
    \end{tikzpicture}
  \caption{Diverse ensemble design for autoencoders. (a) Fully connected networks, (b) Randomly dropped connections, and (c) Connections chosen using a data-driven approach.}
  \label{fig:ensembleConnections}
\end{figure}

\begin{figure}[ht!]
\small
  \begin{center}
     \begin{tikzpicture}
      \begin{axis}[
        ybar,
        width=\linewidth,
        height=0.6*\axisdefaultheight,
    	ylabel={},
    	yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5},
        scaled y ticks=false,
        symbolic x coords={\textit{Precision},\textit{Recall},\textit{F1},\textit{ROC},\textit{PR}},
        xtick=data,
        xtick align=inside,
    	enlargelimits=0.2,
    	legend style={at={(0.5,-0.25)},
    	anchor=north,legend columns=-1}]
        \addplot coordinates {(\textit{Precision},0.832854504) (\textit{Recall},0.944297719) (\textit{F1},0.898096924) (\textit{ROC},0.641887336) (\textit{PR},0.78364474)};
        \addplot coordinates {(\textit{Precision},0.813291419) (\textit{Recall},0.93997599) (\textit{F1},0.870635433) (\textit{ROC},0.589346655) (\textit{PR},0.769615861)};
        \legend{Clean,Dirty}
       \end{axis}
    \end{tikzpicture}
  \end{center}
  \caption{{\color{red}Effect of Datasets, \textit{HRSS}.}}%Effect on metrics of using a clean data and dirty data during the training stage.}
  \label{fig:thresholdChoice}
\end{figure}

==> tables/Ablation_ECG.tex <==
\begin{table}[ht!]
    \small
    \centering
    %\vspace{-1pt}
    \caption{Ablation study, \textit{ECG}.}
    %\vspace{-10pt}
    \label{table:ECGAblation}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{No attention} & 0.1440 & 0.4809 & 0.1840 & 0.1037 & 0.5606 \\
\texttt{No diversity} & 0.1683 & 0.4714 & 0.1819 & 0.1244 & \textbf{0.5939} \\
\texttt{No ensemble} & 0.1919 & 0.4574 & 0.1954 & 0.1297 & 0.5633 \\
\texttt{No re-scaling} & 0.1806 & 0.4819 & 0.1741 & 0.1130 & 0.5379 \\
\texttt{\texttt{CAE-Ensemble}} & \textbf{0.2522} & \textbf{0.4924} & \textbf{0.2521} & \textbf{0.1887} & 0.5715 \\
        \hline
    \end{tabular}
    %\vspace{-1em}
\end{table}

==> tables/Ablation_SMAP.tex <==
\begin{table}[ht!]
    \small
    \centering
    %\vspace{-1pt}
    \caption{Ablation study, \textit{SMAP}.}
    %\vspace{-10pt}
    \label{table:SMAPAblation}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{No attention} & 0.3290 & 0.5763 & 0.3049 & 0.1957 & 0.5605 \\
\texttt{No diversity} & 0.3241 & 0.5841 & 0.3210 & 0.2186 & 0.5832 \\
\texttt{No ensemble} & 0.3175 & 0.5912 & 0.3170 & 0.2135 & 0.5892 \\
\texttt{No re-scaling} & 0.3252 & 0.5689 & 0.2872 & 0.1938 & 0.5666 \\
\texttt{\texttt{CAE-Ensemble}} & \textbf{0.3387} & \textbf{0.6187} & \textbf{0.3327} & \textbf{0.2223} & \textbf{0.6080} \\
        \hline
    \end{tabular}
    %\vspace{-1em}
\end{table}

==> tables/Accuracy_ECG.tex <==
\begin{table}[ht!]
    \small
    \centering
    %\vspace{-1pt}
    \caption{\textit{ECG} accuracy results.}
    %\vspace{-10pt}
    \label{table:ECG}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{ISF} & 0.0543 & \textbf{0.7199} & 0.0999 & 0.0501 & 0.5062 \\
\texttt{LOF} & 0.0539 & 0.6539 & 0.0962 & 0.0500 & 0.4912 \\
\texttt{MAS} & 0.0670 & 0.6276 & 0.1159 & 0.0578 & 0.5342 \\
\texttt{OCSVM} & 0.0825 & 0.4987 & 0.1309 & 0.0588 & 0.5342 \\
        \hline
\texttt{MSCRED} & 0.1789 & \underline{0.6651} & \underline{0.2303} & 0.1055 & 0.5166 \\
\texttt{OMNIANOMALY} & \underline{0.2220} & 0.4938 & 0.2042 & \underline{0.1409} & 0.5584 \\
\texttt{RNNVAE} & 0.1768 & 0.4222 & 0.1439 & 0.0895 & 0.5500 \\
\texttt{AE-Ensemble} & 0.1583 & 0.5398 & 0.1907 & 0.1302 & \textbf{0.5952} \\
\texttt{RAE} & 0.1297 & 0.5394 & 0.1669 & 0.0936 & \underline{0.5922} \\
\texttt{RAE-Ensemble} & 0.2003 & 0.5838 & 0.1864 & 0.1176 & 0.5372 \\
        \hline
\texttt{CAE} & 0.1919 & 0.4574 & 0.1954 & 0.1297 & 0.5633 \\
\texttt{CAE-Ensemble} & \textbf{0.2522} & 0.4924 & \textbf{0.2521} & \textbf{0.1887} & 0.5715 \\
        \hline
    \end{tabular}
    %\vspace{-1em}
\end{table}

==> tables/Accuracy_MSL.tex <==
\begin{table}[ht!]
    \small
    \centering
    %\vspace{-1pt}
    \caption{\textit{MSL} accuracy results.}
    %\vspace{-10pt}
    \label{table:MSL}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{ISF} & 0.1553 & 0.6512 & 0.1895 & 0.1085 & 0.5036 \\
\texttt{LOF} & 0.2463 & 0.5316 & 0.2358 & 0.1431 & 0.5268 \\
\texttt{MAS} & \textbf{0.2959} & 0.5537 & 0.2525 & 0.1595 & 0.5469 \\
\texttt{OCSVM} & \underline{0.2847} & 0.5149 & 0.2616 & 0.1581 & 0.5629 \\
        \hline
\texttt{MSCRED} & 0.1243 & \textbf{0.7747} & 0.1874 & 0.1166 & 0.5072 \\
\texttt{OMNIANOMALY} & 0.1936 & 0.6297 & 0.2414 & 0.1609 & 0.5429 \\
\texttt{RNNVAE} & 0.1641 & 0.5639 & 0.2125 & 0.1378 & 0.5335 \\
\texttt{AE-Ensemble} & 0.1775 & \underline{0.6936} & 0.2424 & 0.1404 & 0.5360 \\
\texttt{RAE} & 0.2069 & 0.6091 & 0.2423 & 0.1503 & 0.5575 \\
\texttt{RAE-Ensemble} & 0.2085 & 0.5633 & 0.2495 & 0.1572 & 0.5714 \\
        \hline
\texttt{CAE} & 0.2223 & 0.5273 & \underline{0.2649} & \textbf{0.1641} & \underline{0.5843} \\
\texttt{CAE-Ensemble} & 0.2501 & 0.5343 & \textbf{0.2713} & \underline{0.1633} & \textbf{0.5963} \\
        \hline
    \end{tabular}
    %\vspace{-1em}
\end{table}

==> tables/Accuracy_Overall.tex <==
\begin{table}[ht!]
    \small
    \centering
    %\vspace{-1pt}
    \caption{Overall accuracy results.}
    %\vspace{-10pt}
    \label{table:Overall}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{ISF} & 0.1008 & \underline{0.5669} & 0.1426 & 0.0818 & 0.5078 \\
\texttt{LOF} & 0.1698 & 0.4552 & 0.1661 & 0.1025 & 0.5233 \\
\texttt{MAS} & 0.2751 & 0.4528 & 0.2377 & 0.1714 & 0.5870 \\
\texttt{OCSVM} & 0.2125 & 0.4351 & 0.2065 & 0.1350 & 0.5487 \\
        \hline
\texttt{MSCRED} & 0.1262 & \textbf{0.7781} & 0.1913 & 0.0927 & 0.5274 \\
\texttt{OMNIANOMALY} & 0.2378 & 0.4952 & 0.2530 & 0.1560 & 0.5965 \\
\texttt{RNNVAE} & 0.2449 & 0.4370 & 0.2289 & 0.1521 & 0.5722 \\
\texttt{AE-Ensemble} & 0.2404 & 0.4727 & 0.2379 & 0.1498 & 0.6078 \\
\texttt{RAE} & 0.2365 & 0.4867 & 0.2406 & 0.1549 & 0.5747 \\
\texttt{RAE-Ensemble} & \underline{0.2875} & 0.4786 & 0.2585 & 0.1719 & 0.6063 \\
        \hline
\texttt{CAE} & 0.2858 & 0.4516 & \underline{0.2735} & \underline{0.1923} & \underline{0.6156} \\
\texttt{CAE-Ensemble} & \textbf{0.3668} & 0.4438 & \textbf{0.3037} & \textbf{0.2180} & \textbf{0.6231} \\
        \hline
    \end{tabular}
    %\vspace{-1em}
\end{table}

==> tables/Accuracy_SMAP.tex <==
\begin{table}[ht!]
    \small
    \centering
    %\vspace{-1pt}
    \caption{\textit{SMAP} accuracy results.}
    %\vspace{-10pt}
    \label{table:SMAP}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{ISF} & 0.1396 & 0.5298 & 0.1986 & 0.1300 & 0.4979 \\
\texttt{LOF} & 0.2261 & 0.5178 & 0.2027 & 0.1289 & 0.5005 \\
\texttt{MAS} & 0.2819 & 0.5174 & 0.2542 & 0.1655 & 0.5233 \\
\texttt{OCSVM} & 0.2561 & 0.5722 & 0.2302 & 0.1461 & 0.4924 \\
        \hline
\texttt{MSCRED} & 0.1266 & \textbf{0.8199} & 0.1914 & 0.1028 & 0.4403 \\
\texttt{OMNIANOMALY} & 0.2307 & 0.6222 & 0.2681 & 0.1556 & 0.5402 \\
\texttt{RNNVAE} & 0.1622 & 0.5646 & 0.1971 & 0.1192 & 0.5119 \\
\texttt{AE-Ensemble} & 0.3134 & 0.5895 & 0.2939 & 0.1780 & 0.5496 \\
\texttt{RAE} & 0.2071 & 0.6316 & 0.2381 & 0.1476 & 0.5390 \\
\texttt{RAE-Ensemble} & 0.2603 & \underline{0.6604} & 0.2529 & 0.1628 & 0.5716 \\
        \hline
\texttt{CAE} & \underline{0.3175} & 0.5912 & \underline{0.3170} & \underline{0.2135} & \underline{0.5892} \\
\texttt{CAE-Ensemble} & \textbf{0.3387} & 0.6187 & \textbf{0.3327} & \textbf{0.2223} & \textbf{0.6080} \\
        \hline
    \end{tabular}
    %\vspace{-1em}
\end{table}

==> tables/Accuracy_SMD.tex <==
\begin{table}[ht!]
    \small
    \centering
    %\vspace{-1pt}
    \caption{\textit{SMD} accuracy results.}
    %\vspace{-10pt}
    \label{table:SMD}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{ISF} & 0.0880 & \underline{0.4571} & 0.1079 & 0.0591 & 0.5066 \\
\texttt{LOF} & 0.2494 & 0.2571 & 0.1764 & 0.1203 & 0.5695 \\
\texttt{MAS} & \underline{0.4720} & 0.4099 & 0.3716 & \underline{0.3253} & \textbf{0.7520} \\
\texttt{OCSVM} & 0.3414 & 0.2944 & 0.2626 & 0.1927 & 0.5783 \\
        \hline
\texttt{MSCRED} & 0.0631 & \textbf{0.7719} & 0.1100 & 0.0395 & 0.5000 \\
\texttt{OMNIANOMALY} & 0.2432 & 0.3328 & 0.2110 & 0.1503 & 0.6148 \\
\texttt{RNNVAE} & 0.4334 & 0.3194 & 0.3045 & 0.2406 & 0.6917 \\
\texttt{AE-Ensemble} & 0.3713 & 0.3709 & 0.2832 & 0.2349 & 0.6823 \\
\texttt{RAE} & 0.4466 & 0.3037 & 0.3078 & 0.2424 & 0.6836 \\
\texttt{RAE-Ensemble} & 0.4684 & 0.3318 & 0.3332 & 0.2639 & 0.6998 \\
        \hline
\texttt{CAE} & 0.4625 & 0.3804 & \textbf{0.3895} & \textbf{0.3299} & \underline{0.7416} \\
\texttt{CAE-Ensemble} & \textbf{0.4924} & 0.3739 & \underline{0.3770} & 0.3246 & 0.7375 \\
        \hline
    \end{tabular}
    %\vspace{-1em}
\end{table}

==> tables/Accuracy_SWaT.tex <==
\begin{table}[ht!]
    \small
    \centering
    \caption{\textit{SWaT} accuracy results. {\color{red} Include it?}}
    \label{table:SWaT}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{ISF} & 0.1390 & 0.2491 & 0.1524 & 0.1268 & 0.5005 \\
\texttt{LOF} & 0.1224 & 0.9753 & 0.1483 & 0.1144 & 0.4838 \\
\texttt{MAS} & 0.1215 & \textbf{1.0000} & 0.1474 & 0.0786 & 0.2272 \\
\texttt{OCSVM} & 0.1343 & 0.9172 & 0.1620 & 0.0901 & 0.3457 \\
        \hline
\texttt{AE-Ensemble} & \textbf{0.9960} & 0.5946 & \textbf{0.8775} & 0.7407 & \textbf{0.8490} \\
\texttt{MSCRED} & 0.1574 & 0.1031 & 0.1424 & 0.0695 & 0.5540 \\
\texttt{OMNIANOMALY} & 0.9951 & 0.5955 & 0.8773 & 0.6983 & 0.8123 \\
\texttt{RNNVAE} & 0.1712 & 0.8259 & 0.2034 & 0.1629 & 0.6311 \\
\texttt{RAE} & 0.9957 & 0.5490 & 0.8563 & \textbf{0.7470} & 0.8420 \\
\texttt{RAE-Ensemble} & 0.9774 & 0.5783 & 0.8589 & 0.7463 & 0.8488 \\
        \hline
\texttt{CAE} & 0.5127 & 0.5724 & 0.5236 & 0.3848 & 0.7634 \\
\texttt{CAE-Ensemble} & 0.8013 & 0.6083 & 0.7534 & 0.6513 & 0.8358 \\
        \hline
    \end{tabular}
\end{table}

==> tables/Accuracy_WADI.tex <==
\begin{table}[ht!]
    \small
    \centering
    %\vspace{-1pt}
    \caption{\textit{WADI} accuracy results.}
    %\vspace{-10pt}
    \label{table:WADI}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{PR}  & \textit{ROC} \\ 
        \hhline{|=||=|=|=|=|=|}
\texttt{ISF} & 0.0667 & \underline{0.4765} & 0.1170 & 0.0610 & 0.5248 \\
\texttt{LOF} & 0.0736 & 0.3155 & 0.1193 & 0.0702 & 0.5284 \\
\texttt{MAS} & 0.2586 & 0.1555 & 0.1942 & 0.1490 & 0.5788 \\
\texttt{OCSVM} & 0.0980 & 0.2955 & 0.1472 & 0.1192 & 0.5754 \\
        \hline
\texttt{MSCRED} & 0.1382 & \textbf{0.8590} & 0.2377 & 0.0993 & \underline{0.6730} \\
\texttt{OMNIANOMALY} & 0.2996 & 0.3976 & \textbf{0.3404} & 0.1723 & \textbf{0.7261} \\
\texttt{RNNVAE} & 0.2881 & 0.3147 & \underline{0.2867} & \underline{0.1734} & 0.5739 \\
\texttt{AE-Ensemble} & 0.1619 & 0.2398 & 0.1928 & 0.0911 & 0.5102 \\
\texttt{RAE} & 0.2118 & 0.2799 & 0.2342 & 0.1150 & 0.6667 \\
\texttt{RAE-Ensemble} & \underline{0.2999} & 0.2535 & 0.2707 & 0.1580 & 0.6516 \\
        \hline
\texttt{CAE} & 0.2350 & 0.3019 & 0.2004 & 0.1243 & 0.5994 \\
\texttt{CAE-Ensemble} & \textbf{0.5006} & 0.1995 & 0.2853 & \textbf{0.1911} & 0.6023 \\
        \hline
    \end{tabular}
    %\vspace{-1em}
\end{table}

==> tables/Old_tables.tex <==
\begin{table}[ht!]
    \centering
    \caption{{\color{red}\textit{ECG} accuracy results.}}
    \label{table:ECG}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
         \texttt{IS} & 0.2857 & 0.2857 & 0.2857 & 0.4438 & 0.0562 \\
         \texttt{LOF} & 0.2857 & 0.2852 & 0.2854 & 0.4708 & 0.0468 \\
         \texttt{SVM} & 0.5714 & 0.5701 & 0.5708 & 0.3979 & 0.0483 \\
        \hline
         \texttt{RAE} & 0.7233 & 0.9954 & 0.7854 & 0.4386 & 0.0849 \\
         \texttt{CAE} & 0.6858 & 0.9933 & 0.8070 & 0.5280 & 0.1011 \\
         \texttt{DAGMM} & 0.8064 & 0.9942 & 0.8905 & 0.4944 & 0.0512 \\
         \texttt{MSCRED} & 0.7657 & 0.7143 & 0.7391 & 0.5054 & 0.1054 \\
         \texttt{RAE-Ensemble} & 0.8128 & 0.9954 & 0.8889 & 0.5285 & 0.1207 \\
        \hline
        \texttt{CAE-Ensemble} & \textbf{0.8290} & \textbf{1.0000} & \textbf{0.8927} & \textbf{0.5546} & \textbf{0.1353} \\
        \hline
    \end{tabular}
\end{table}


\begin{table}[ht!]
    \centering
    \caption{{\color{red}\textit{SMD} accuracy results.}}
    \label{table:SMD}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \texttt{IS} & 0.3813 & \textbf{0.9800} & 0.4825 & 0.1724 & 0.0242 \\
        \texttt{LOF} & 0.4704 & 0.8949 & 0.5595 & 0.4347 & 0.0384 \\
        \texttt{SVM} & 0.5453 & 0.9758 & 0.6394 & 0.5153 & 0.1262 \\
        \hline
        \texttt{RAE} & 0.5233 & 0.5393 & 0.4976 & 0.6358 & 0.2266 \\
        \texttt{CAE} & 0.9215 & 0.9094 & \textbf{0.9010} & 0.8052 & 0.3777 \\
        \texttt{DAGMM} & 0.5900 & 0.6476 & 0.6063 & 0.4992 & 0.0422 \\
        \texttt{MSCRED} & 0.8830 & 0.8602 & 0.8714 & 0.4299 & 0.0595 \\
        \texttt{RAE-Ensemble} & 0.8529 & 0.8596 & 0.8562 & 0.6723 & 0.2905 \\
        \hline
        \texttt{CAE-Ensemble} & \textbf{0.9301} & 0.8790 & 0.8762 & \textbf{0.8241} & \textbf{0.3970} \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{{\color{red}\textit{Donut} accuracy results.}}
    \label{table:Donut}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \texttt{IS} & 0.0820 & 0.5093 & 0.1375 & 0.2313 & 0.0081 \\
        \texttt{LOF} & 0.0223 & 0.2745 & 0.0413 & 0.4721 & \textbf{0.1736} \\
        \texttt{SVM} & 0.1283 & 0.3818 & 0.1921 & 0.2406 & 0.0100 \\
        \hline
        \texttt{RAE} & 0.1667 & 0.0718 & 0.1003 & 0.6060 & 0.0281 \\
        \texttt{CAE} & 0.0176 & 0.1440 & 0.0311 & 0.7201 & 0.0976 \\
        \texttt{DAGMM} & 0.1158 & \textbf{0.6936} & 0.1984 & 0.4952 & 0.0150 \\
        \texttt{RAE-Ensemble} & \textbf{0.4798} & 0.1758 & 0.2438 & 0.7305 & 0.0848 \\
        \hline
        \texttt{CAE-Ensemble} & 0.2417 & 0.3216 &  \textbf{0.2758} &  \textbf{0.7638} & 0.1302 \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{\textit{AIOps} accuracy results.}
    \label{table:AIOps}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} & \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \texttt{IS} & 0.9880 & 0.9032 & 0.9433 & 0.9267 & 0.9973 \\
        \texttt{LOF} & 0.9879 & 0.9725 & 0.9796 & 0.8524 & 0.9879 \\
        \texttt{SVM} & \textbf{0.9994} & 0.5148 & 0.6785 & 0.9312 &\textbf{0.9989} \\
        \hline
        \texttt{RAE} & 0.9985 & 0.9826 & 0.9904 & \textbf{0.9541} & 0.9900 \\
        \texttt{DAGMM} & 0.7135 & 0.7956 & 0.7545 & 0.6114 & 0.9705 \\
        \texttt{RAE-Ensemble} & 0.9802 & 0.9481 & 0.9639 & 0.5173 & 0.9742 \\
        \hline
        \texttt{CAE (Ours)} & 0.9942 & \textbf{0.9994} & \textbf{0.9968} & 0.8725 & 0.9863 \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{{\color{red}\textit{Yahoo} accuracy results.}}
    \label{table:Yahoo}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \texttt{IS} & 0.3376 & 0.4192 & 0.3574 & 0.0704 & 0.0044 \\
        \texttt{LOF} & 0.2643 & 0.2790 & 0.2678 & 0.3131 & 0.0205 \\
        \texttt{SVM} & 0.5443 & 0.5610 & 0.5086 & 0.4041 & 0.1981 \\
        \hline
        \texttt{RAE} & 0.5146 & 0.6268 & 0.4368 & 0.8602 & 0.5403 \\
        \texttt{CAE} & 0.4194 & 0.4908 & 0.4393 & 0.7558 & 0.5751 \\
        \texttt{DAGMM} & 0.4405 & 0.5344 & 0.4829 & 0.4812 & 0.0094 \\
        \texttt{RAE-Ensemble} & 0.5233 & 0.5393 & 0.4976 & 0.8601 & 0.6826 \\
        \hline
        \texttt{CAE-Ensemble} & \textbf{0.6593} & \textbf{0.6630} & \textbf{0.6530} & \textbf{0.9212} & \textbf{0.7805} \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{{\color{red}Overall accuracy results.}}
    \label{table:Overall}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Model} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \texttt{IS} & 0.2717 & 0.5485 & 0.3158 & 0.2295 & 0.0232 \\
        \texttt{LOF} & 0.2607 & 0.4334 & 0.2885 & 0.4227 & 0.0698 \\
        \texttt{SVM} & 0.4473 & 0.6222 & 0.4777 & 0.3895 & 0.0956 \\
        \hline
        \texttt{RAE} & 0.4820 & 0.5583 & 0.4550 & 0.6352 & 0.2200 \\
        \texttt{CAE} & 0.5111 & 0.6344 & 0.5446 & 0.7023 & 0.2879 \\
        \texttt{DAGMM} & 0.4882 & 0.7097 & 0.5445 & 0.4925 & 0.0294 \\
        \texttt{RAE-Ensemble} & \textbf{0.6672} & 0.6425 & 0.6216 & 0.6978 & 0.2946 \\
        \hline
        \texttt{CAE-Ensemble} & 0.6650 & \textbf{0.7159} & \textbf{0.6744} & \textbf{0.7659} & \textbf{0.3607} \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{Ablation study, \textit{Yahoo}.}
    \label{table:YahooAblation}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{\texttt{CAE-Ensemble}} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \textit{No attention} & 0.9941 & 0.9852 & 0.9896 & 0.7087 & 0.9905 \\
        \textit{No transfer} & 0.9911 & 0.9922 & 0.9916 & 0.7360 & 0.9877 \\
        \textit{No ensemble} & 0.9936 & 0.9943 & 0.9939 & 0.6577 & 0.9939 \\
        \textit{Fixed threshold} & 0.9938 & 0.9799 & 0.9867 & \textbf{0.9396} & \textbf{0.9990} \\
        \textit{Complete model} & \textbf{0.9961} & \textbf{0.9992} &   \textbf{0.9977} & \textbf{0.9396} & \textbf{0.9990} \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{Ablation study, \textit{ECG}.}
    \label{table:ECGAblation}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{\texttt{CAE-Ensemble}} &  \textit{Precision} &  \textit{Recall} &  \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \textit{No attention} & \textbf{0.9540} & 0.9668 & 0.9603 & 0.6319 & 0.9452 \\
        \textit{No transfer} & 0.9517 & 0.9928 & 0.9717 & 0.6685 & 0.9530 \\
        \textit{No ensemble} & 0.9516 & 0.9914 & 0.9711 & 0.5324 & \textbf{0.9633} \\
        \textit{Fixed threshold} & 0.9520 & 0.9819 & 0.9666 & \textbf{0.6707} & 0.9394 \\
        \textit{Complete model} & 0.9523 & \textbf{0.9935} & \textbf{0.9724} & \textbf{0.6707} & 0.9394 \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{Input settings sensitivity, \textit{Yahoo}.}
    \label{table:SensitiveYahoo}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Size} &  \textit{Precision} &  \textit{Recall} &     \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \textit{Single series} & \textbf{0.9961} & 0.9988 & 0.9975 & 0.8020 & 0.9954 \\
        \textit{NGram 64} & \textbf{0.9961} & 0.9935 & 0.9948 & 0.6824 & 0.9966 \\
        \textit{NGram 128} & \textbf{0.9961} & 0.9977 & 0.9969 & 0.6893 & 0.9965 \\
        \textit{NGram 256} & \textbf{0.9961} & 0.9983 & 0.9972 & 0.7472 & 0.9985 \\
        \textit{Batch 128} & \textbf{0.9961} & \textbf{0.9992} &    \textbf{0.9977} & \textbf{0.9396} & \textbf{0.9990} \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{Input settings sensitivity, \textit{ECG}.}
    \label{table:SensitiveECG}
    \begin{tabular}{ |l||c|c|c|c|c| } 
        \hline
        \textbf{Size} &  \textit{Precision} &  \textit{Recall} &     \textit{F1} & \textit{ROC}  & \textit{PR} \\ 
        \hhline{|=||=|=|=|=|=|}
        \textit{Single series} & 0.9500 & 0.9585 & 0.9542 & 0.5320 & 0.9588 \\
        \textit{NGram 64} & 0.9514 & 0.9877 & 0.9692 & 0.6021 & 0.9717 \\
        \textit{NGram 128} & 0.9520 & 0.9622 & 0.9571 & \textbf{0.6928} & 0.9679 \\
        \textit{NGram 256} & 0.9502 & 0.9624 & 0.9563 & 0.6264 &    \textbf{0.9744} \\
        \textit{Batch 128} &\textbf{0.9523} & \textbf{0.9935} &    \textbf{0.9724} & 0.6707 & 0.9394 \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[ht!]
\centering
\caption{Autoencoder-based models for outlier detection.}
\label{table:summary}
\begin{tabular}{c|P{1.4cm}|c|c|}
\cline{2-4}
& \textit{Temporal-dependencies} 
& \textit{Diversity} & \textit{Efficiency} \\ \hline
\multicolumn{1}{|l|}{\texttt{AE}} & \xmark  & \xmark & \cmark \\ \hline
\multicolumn{1}{|l|}{\texttt{RAE}} & \cmark & \xmark & \xmark \\ \hline
\multicolumn{1}{|l|}{\texttt{CAE}} & \cmark & \xmark & \cmark \\ \hline
\multicolumn{1}{|l|}{\texttt{AE-Ensemble}} & \xmark  & \cmark~(Random) & \cmark \\ \hline
\multicolumn{1}{|l|}{\texttt{RAE-Ensemble}} & \cmark  & \cmark~(Random) & \xmark \\ \hline
\multicolumn{1}{|p{1.8cm}|}{\texttt{CAE-Ensemble}} & \cmark & \cmark & \cmark \\ \hline
\end{tabular}
\end{table}

==> tables/Window_MSL.tex <==
\begin{table}[ht!]
    \centering
    \caption{Window size choice, \textit{MSL}.}
    \label{table:WindowMSL}
    \begin{tabular}{ |l||c|c|c| } 
        \hline
        \textbf{Window} &  \textit{Validation error} &  \textit{PR} & \textit{ROC} \\ 
        \hhline{|=||=|=|=|}
        \textit{4} & 1268.54 & 0.1589 & 0.5724 \\
        \textit{32} & 1315.14 & 0.1667 & \textbf{0.6024} \\
        \textit{128} & 1362.34 & 0.1714 & 0.5862 \\
        \textbf{16 - Median} & 1420.73 & 0.1641 & 0.5843 \\
        \textit{64} & 1547.48 & 0.1539 & 0.5767 \\
        \textit{8} & 1588.91 & 0.1639 & 0.6015 \\
        \textit{256} & 1620.40 & \textbf{0.1735} & 0.5641 \\
        \hline
    \end{tabular}
\end{table}

==> tables/Window_WADI.tex <==
\begin{table}[ht!]
    \centering
    \caption{Window size choice, \textit{WADI}.}
    \label{table:WindowWADI}
    \begin{tabular}{ |l||c|c|c| } 
        \hline
        \textbf{Window} &  \textit{Validation error} &  \textit{PR} & \textit{ROC} \\ 
        \hhline{|=||=|=|=|}
        \textit{16} & 246.78 & 0.1851 & \textbf{0.6829} \\
        \textit{4} & 283.44 & 0.1732 & 0.5243 \\
        \textit{8} & 339.66 & 0.1753 & 0.5979 \\
        \textbf{32- Median} & 341.31 & 0.1911 & 0.6023 \\
        \textit{64} & 1177.85 & \textbf{0.2046} & 0.6690 \\
        \textit{256} & 1619.29 & 0.1656 & 0.5548 \\
        \textit{128} & 5746.66 & 0.1558 & 0.5984 \\
        \hline
    \end{tabular}
\end{table}

